Perception of Deepfakes among Bangladeshi Women

As deepfake technology becomes more accessible, concerns about its misuse and societal impact are escalating, particularly in regions like the Global South where digital literacy and regulatory measures are often limited. While previous research has explored deepfakes in contexts such as detection and media manipulation, there is a noticeable gap in understanding how individuals in these regions perceive and interact with deepfake media. This study addresses this gap by investigating how Bangladeshi women perceive deepfakes and the socio-cultural factors influencing their awareness, concerns, and responses to this technology. Drawing on 15 semi-structured interviews, we uncover how cultural values, gendered norms, trust in institutions, and the prevalence of digital harassment shape their perceptions and coping mechanisms. Through this research, we aim to advance existing scholarship in HCI by offering insights into the design of culturally sensitive interventions, educational initiatives, and policy frameworks to address the challenges posed by deepfakes in the Global South.

==> find-old.tex <==
\section{Findings}

We first present a vignette to portray the experiences of deepfake abuse by Bangladeshi women. This story is from one of our participants, Riya (pseudonym).\\

\textit{Riya (23) is a university student in Rajshahi. She is actively engaged in several voluntary student organizations. Due to her outspoken presence, she gained a lot of visibility among her peers. In her senior year, just before the election of the new student committee in one of the organizations, some of her peers circulated some sexually explicit images across the student networks. Her face was manipulated in those images. The content quickly spread through social media; even among her friends and relatives. Riya was pressured to resign from all the student organizations she was affiliated with. When her parents got to know about this, they were furious. Her mother told her to quit studies and leave the campus. Riya wants to ask for legal help, but she says that the police can't do anything to find the perpetrators. She also fears that filing a formal complaint might attract media attention and it can get more widespread. She's also scared that if the perpetrators come to know about her legal steps, they might do more harm to her.}\\

This story resonated with the experiences of all our participants who faced deepfake-related abuse. It describes the multi-layered harms caused by deepfake technologies when weaponized against women in conservative socio-cultural contexts like Bangladesh.

% This deepfake content goes beyond the digital space to impact their educational, social, and familial life. It not only alters the societal image they build over the years, also erases them from all the public and institutional spaces they once occupied.

In the following section, we detail the perceptions and concerns of Bangladeshi women about deepfake technologies. We also report the preventive measures they adopt to safeguard their privacy.

% We organize the findings into five key themes: (1) Familiarity and Perception, (2) gendered and cultural vulnerabilities, (3) verification practices, (4) privacy strategies, (5) legal and moral considerations. Each theme is explored in detail below.

\subsection{Deepfake? It's never fun!}
Although in some cases deepfake might be perceived as an entertaining technology, our participants shared that the ``idea of manipulating videos and images" as ``scary", ``harmful", ``risky", and ``dangerous" to them. 

P7 described deepfakes as more like a ``weapon" than a mode of entertainment or fun:

\begin{quote} Nowadays, people use deepfakes to poke fun at or bully someone, to harass them, or even to create political controversy. It’s almost like a weapon, a lot of individuals are targeted this way. For me, the concept of deepfakes has taken on a negative connotation. This can never be fun!\end{quote}

P5 expressed that she isn't comfortable with any deepfake use of her photo, even by friends, because she fears it could be shared or misused anytime regardless of the original intent, 

\begin{quote} Whatever the purpose may be, I cannot allow my photo to be used in any [deepfake] content. Even if they say it will only be kept between us, I can't trust that eventually it won't be spread or shared. It could start from a simple argument between us or be passed around ``just for fun!" Everyone can use it as a source of entertainment to get views. I'm not comfortable with that (...) Never up for any kind of deepfake fun, not even with my friends. \end{quote}

The concerns expressed by P5 and P7 regarding the fear of being targeted were echoed in the stories of other participants. P14 (24), who experienced deepfake abuse, recounted how this type of content shared with her intimate partner was later used against her,

% P5 and P7's fear of being targeted was reflected in the experiences of our other particpants. P3 (24), who was a victim of deepfake abuse, shared her story how a fun content shared with her intimate partner backstabbed her:

\begin{quote} In my previous relationship, my boyfriend and I used to make fun intimate videos of us using an app called Luma. They were like kissing videos, hugging videos, etc. Unfortunately that relationship didn’t work out. (...) After we broke up and I got married, he sent those intimate videos to my husband. It was so embarrassing and humiliating! I was terrified it might lead to a divorce. I had just gotten married, and it was deeply traumatic for both me and my husband. I felt completely helpless. I never imagined he would use something so personal out of revenge. This is insane!\end{quote}

P8 also described how her friend was harassed by her ex-boyfriend who circulated her sexually explicit deepfake images online after their breakup,

\begin{quote} One of my friends broke up with her boyfriend and created an expose post about how he had tortured her. Later, when they broke up, he manipulated her photos using AI, and replaced her images with something else [sexually explicit content]. He shared those manipulated content on social media to bully her.\end{quote}

P6 recounted a similar incident which happened to her cousin, an Instagram influencer,

\begin{quote} 
A very viral piece of content was released on social media where her face was taken from a picture and used in a pornographic video. The perpetrator turned out to be someone from her follower list. That guy wanted to start a romantic relationship with her. When she refused, this incident occurred. 
\end{quote}






% Despite the increasing misuse of deepfakes, conversations around their ethical implications remain superficial. Participants said that such discussions often trivialize the risks, and it focuses instead on the novelty of the technology rather than its potential for harm:

% \begin{quote} We talk about how easy it is to make a kissing video, but not about the safeguarding issues. These aren’t impactful conversations. We talk about the harmful side of deepfakes in a funny or joking way—like, "Look at what people are doing these days!" or "Check out what I can do with this app." But we rarely address the ethical or moral aspects in our discussions. \end{quote}

% One participant emphasized that limited education, technical literacy, and awareness exacerbate the potential for deepfake-related abuse and harm:

% \begin{quote} In the context of Bangladesh, those of us who have access to the internet and the technical skills to use apps and create content are often not educated about using these tools responsibly. We lack understanding of privacy, consent, and ethical behavior in cyberspace. This gap in awareness and thought processes means we are not prepared to handle these technologies. We don’t fully understand concepts like consent, privacy, or the distinction between ethical and unethical behavior. \end{quote}

% This lack of education and awareness contributes significantly to the misuse of deepfakes, as demonstrated by incidents of abuse that participants recounted.

\subsection{Understanding the Fear: Deepfakes, Gender, and Cultural Trauma}

To understand why our participants consistently described deepfakes as “scary,” it is necessary to situate such fears within the broader sociocultural and gendered landscape of Bangladesh. In this section, we present participants’ reflections on what it means to be a woman in the patriarchal context of Bangladeshi society and how public dissemination of sexually explicit deepfake content can trigger severe consequences for them, such as social ostracization, victim-blaming, and reputational damage.

When talking about how vulnerable women are to deepfake-related harms in a male-dominated society, P7 said,

\begin{quote}
     Women have the pressure to maintain a very good reputation in our society rather than men. If a deepfake content of a girl gets viral, instantly everyone thinks that the girl must be `bad'. They will pick it up, share it among themselves, and keep bringing it up in every situation. But if it's a boy, they will say, ``Oh he is just a boy, let it go!". I have seen a lot of these happening around me.  It's not like this does not happen to the men, but when it happens with a girl it leaves a hundred times worse impact on her life.
\end{quote}

Our other participants also shared that people often feel entitled to say whatever they want about a woman. What felt most upsetting to them was how easily others believed the gossip without questioning whether it was true. P13 added,

\begin{quote}
    In our society, a woman’s reputation is very fragile. People often feel entitled to say whatever they want about her, like just throwing in an extra line to demean her. And the worst part is people believe it without question. It’s almost instantly accepted, “Oh, she must’ve done it.” Or they'll be like, ``Why would a woman use social media?" These kinds of things are far too common here; it’s just too easy to point a finger at a woman.
\end{quote}

When a deepfake content is spread, it is extremely hard to self-explain to family members because it's considered taboo to talk about it with others for a girl, especially her parents or family members. P10 said,

\begin{quote}
   If something like this ever happened to me, how would I even talk to my parents about it? In our culture, topics like these are so taboo, we’re not supposed to speak about them with our parents or elders. It feels inappropriate, even shameful (...) and if I can’t talk about it, how would I even begin to explain what happened? How would they ever understand?
\end{quote}

\victimblaming

P13's concerns were reflected in P8's experience of how she was victimized when her deepfake content was made public. She recounted,

\begin{quote}
    [When my parents got to know about this] they were like, ``Did you really do this? Be truthful, did you? We don't know anything, you must be lying!"
\end{quote}

P6 added how this situation can affect the victim's family members' reputation in the society as well,

\begin{quote}
    If a girl ever faces any deepfake-related abuse, the question is always raised against her, ``Why would someone do this to her? She must have done something bad (...)'' Not only that, when the neighborhood gets to know about this, her family gets pressurized to control their daughter, ``Why don't you control her? What kind of parents you are?"
\end{quote}

P11 shared how her sister was forced to leave her hometown after going through a similar situation,

\begin{quote}
    She [her sister] was very active on social media and some people used her social media photos and manipulated them. They made some distorted photos, and circulated that this girl was involved in various inappropriate activities. Her parents couldn't keep their daughter in that area and shifted to Dhaka. 
\end{quote}

% To understand why our participants moved beyond simplistic notions of “online fun” to describe deepfakes, we need to situate deepfake harm within their sociocultural context, and unveil ...how the public exposure of deepfake content can trigger severe consequences for women, such as social ostracization, victim-blaming, and reputational damage. These reactions are not isolated but rooted in patriarchal norms that tie a woman’s worth to her perceived sexual purity and public image.  In this section, we will illustrate (after releasing a deepfake video, what a woman faces in the society, family, peers etc.)...to unpack the sociocultural dynamics that shape women’s lives 
% \subsubsection{Sociocultural Perspective towards women}
% 3ta perspective - friends, parents, workplace, society

P4 also pointed out that since everyone uses social media, this kind of content spreads rapidly. As a result, the victim faces even more harassment, abuse, and public humiliation.
When talking about her friend, P8 shared how people reacted in their network after the sexually explicit images of her friend were spread,

\begin{quote}
 I saw how her manipulated pictures became a source of mockery, even among our own friend circles. Even in a simple conversation, this incident became a hot topic! People now make dirty jokes and memes with her photos. Can you imagine how disrespectful it is?
\end{quote}

% It takes a huge toll on her mental health. In the workplace, people talk behind her back, “Did you see what happened to that girl?” These incidents deeply affect not just her personal life, but also her professional reputation and relationships.
P15, a victim of deepfake abuse, shared how her life was `shattered' when her sexually explicit images were made viral by one of her colleagues,

\begin{quote}
    The worst thing was I had to resign from my workplace. My parents were very disappointed, and I couldn't even explain that it was not my image. (...) It was embarrassing to hang out with my friends in public! I felt like I was a disgrace! My life was completely shattered.
\end{quote}

\reputationaldamage

\textbf{(victim BCS er background check e bhoy paay jodi deepfake content chole ashe, corporate job er quote) - later if needed}

These findings reveal that the fear and trauma of deepfakes for women in Bangladesh are not just about the digital manipulation itself, but also about how such content is received and weaponized within a patriarchal culture. However, what makes these harms even more devastating is the limited recourse available to victims. In the next sections, we turn to two structural issues that further compound deepfake-related vulnerabilities: the lack of awareness about deepfakes and digital authentication methods, and the weak legal infrastructure for addressing such abuse.

\subsection{Limited Awareness and Literacy about Deepfakes}

Our participants consistently expressed that most people, including victims themselves, do not understand how deepfakes are created or how to verify the authenticity of such content. For many, this lack of awareness creates confusion, disbelief, and delays in responding to the harm. As P2 said, 

\begin{quote}
    As an NGO worker, I’ve traveled across various regions of Bangladesh and interacted with people from diverse backgrounds. The practice of manipulating images or videos to target and harm certain individuals or groups has existed for years. But most people don’t even know that deepfake content can exist, or that something like this can be made at all.
\end{quote}

P17 added,

\begin{quote}
    Most people, especially the elderly ones and the people in rural areas, don't understand the concept of deepfakes. My parents cannot differentiate between what's manipulated and what's real. Recently AI generated videos have become very popular, and they think these are all real videos. They believe instantly whatever they see. So there's no question of `verifying' or checking the authenticity of the content.
\end{quote}

P13, who is aware of deepfakes, said that she can't identify real or AI-generated images on social media as she's not aware of any verification tools, and sometimes she's not just interested,

\begin{quote}
    A lot of images I see online are personally or emotionally triggering, but I don't understand if they are edited or not. I actually don't always have the head space to check those. And I don't know about any platforms or tools to detect these.
\end{quote}

P9 has an advanced method for verifying content, such as checking the follower number and page likes from where the content has been spread, and checking if the content was shared by any of her trusted contact,

\begin{quote}
    At first I check the source for the authenticity, it can be Facebook page or other platforms. I check their followers and page likes to get an idea if the content might be fake or not. A well known page has way more likes and followers, but actually these pages can also post false information or AI generated pictures. so in that case I check if a known person shared that content or not, and personally ask them if it is true news. I don't know any other way to verify these.
\end{quote}

P15 added that she verified the authenticity of any social media content by checking the public comments,

\begin{quote}
    I check the comment section of the Facebook post to get an idea if the content is fake or not. If it is, then most of the people comment there. 
\end{quote}

For the victims, access to no tools that could prove if her content is fake or not, makes it more tolling. As one of our participants mentioned,

\begin{quote}
    [When my friend's video went viral] people couldn’t tell whether it was real or fake. She knew it was fake, and so did I, but there was no way we could prove it, or no way for others to know.
\end{quote}

P5 said,

\begin{quote}
Such deepfake content, however unrealistic it might be, easily gets spread around. No one checks if that incident really happened or not. They just click on that share button, ``Look, what happened!", and it gets viral on social media. There isn't much scope for verifying this. So many content regarding deepfake is being shared everywhere everyday, now people get annoyed when anyone keeps asking for the source of it.
\end{quote} 

Unlike traditional misinformation, deepfakes are visually convincing and technically sophisticated, which make them much harder to detect through casual observation or social cues. As a result, even those who attempt to verify content may still fall for manipulated media, especially in the absence of digital literacy or formal tools to assess authenticity.


\subsection{Weak Legal Infrastructure}

Despite the severity of deepfake-related harm, most of our participants expressed a hopelessness when it came to seeking legal support. 15 out of 18 of our participants were not aware of any laws which can address these issues. All of our participants felt that the existing laws and the legal system in Bangladesh are not prepared to address deepfake abuse.


P16 expressed concern over the complete lack of legal preparedness:

\begin{quote}
    No, I don’t think they are prepared at all. Deepfake content is being shared openly on platforms like Facebook. No matter what the purpose is, there’s no regulation around it. And if there’s no law, then how are they supposed to handle these cases? What would they even follow? I don’t think anything is being done in this area.
\end{quote}

Several participants shared that even when victims wanted to seek help, they avoided legal steps because they felt it wouldn’t lead to justice and might even make things worse. As one participant noted:

\begin{quote}
    The reason why most girls don’t go to the police is because they know nothing will happen. It’s not just about filing a complaint. You have to keep going back, face questions, get judged. And at the end of all that, no action is taken. So people just stay silent.
\end{quote}

P12 added,

\begin{quote}
    They [the victims] are afraid of going to the police or taking help from the law enforcement. Laws are there but there is no implementation.
\end{quote}

Another participant pointed out that taking legal action could invite even more harassment, including from the authorities themselves,

\begin{quote}
    If you go to the police station and say that your fake video has gone viral, they look at you like it’s your fault. They don’t understand how these things work. Sometimes they even say things like, “Why did you share your photos on social media in the first place?”
\end{quote}

% In Riya’s story (presented at the beginning of this section), we see how fear of retaliation and public exposure keeps victims from seeking justice. Like many others, she worried that filing a case would invite more scrutiny, draw media attention, or provoke the perpetrator to cause further harm.

The absence of a clear legal process, a lack of trained cybercrime officials, and a culture of disbelief and blame discourages women from reporting deepfake abuse. They feel that ``there is no system designed to support them'' when they do.

\subsection{Privacy Strategies to Combat Deepfake-related harm}
Our participants expressed that no privacy strategies such as locking profiles or limiting the information shared on social media can fully protect them from the potential risks of deepfake abuse. P4 said,

\begin{quote} 
    I am breaching my own privacy with my own hands. I have my own website. My photo, my information, these can be seen by everyone out there. Even if I lock my social media profile, I see my photos available in Google search. Anyone can do anything with that!
\end{quote}

Another participant mentioned,

\begin{quote} 
    I think in the world of social media, you can never be fully alert. You always have to be extra cautious. If you’re sharing your photo or your information on a social platform, there’s always some risk of something happening. You cannot be certain that nothing will go wrong, no matter how locked your profile is. If other people have access to your social media, your photo or video can still be easily misused. So, in that case, something like that can easily happen. 
\end{quote}

Another participant said that she wasn't aware of any measures that could save her from such abuse,

\begin{quote}
    We actually don't have any online safety. I don't know how to secure myself so that people cannot access my personal information. We have our photos on Google, we have our socials, we are all over the internet. 
\end{quote}

Some of our participants said that they were concerned sharing personal photos online, but they were also feared of being left out or keeping up with the social trends. P17 (a victim) said,

\begin{quote}
    I frequently travel to different countries, so I post a lot of photos on my socials. I love sharing those with my followers. I know about deepfakes, but I cannot stop doing what I love. My socials are like my digital diary to me.
\end{quote}

P16 said,

\begin{quote}
    Everybody shares their photos on social media. We have a doctors' group, we share our photos there. (...) I often think of this kind of abuses, I also fear this, but the thing is, if I don't keep up with them, my life will seem dull to them and they will talk about it later.
\end{quote}

Five of our participants (including three victims) don't use their real pictures on social media and are extremely cautious about sharing their personal information online. One of them said,

\begin{quote}
    I even fear to use my passport size photo in the job seeking portals, I don't know if they'll do anything with it. (...) In my Facebook, I mostly share memes and reels. I never upload any photo showing my full face.
\end{quote}

P18 added,

\begin{quote}
    My socials are locked, and I only add my family and friends there. One of my friends faced such abuse from a guy from her friendlist, so I try not to add male friends in my Facebook and Instagram.
\end{quote}
% \subsection{Consent and Setting Boundaries}
% When asked about their comfort levels with deepfake content being shared by family members, friends, partners, or strangers, participants expressed strong opinions on the importance of consent and clear boundaries. They were particularly cautious about how and where such content might be shared. For instance, they identified their private spaces as ``family members, maybe my friends, maybe my partner.''

% Participants highlighted that even in private spaces, their comfort levels depended heavily on the closeness of their relationship with the individuals involved:

% \begin{quote} I would not be comfortable at all [if someone uses my photo to create deepfake content]. It can be in a very inner space, like shared in my inbox or in my group chat—to that extent, I think it is fine for me. No problem. But those people have to be very close to me, of course. \end{quote}

% However, their responses became more definitive when discussing the sharing of deepfake content on public platforms. They emphasized the necessity of obtaining explicit consent and expressed their unwillingness to permit such uses.

% But majority of the participants (12 out of 15) stressed that their discomfort extended to the very creation of deepfakes using their likeness, even if consent was sought. For them, the act of creating or using such content was inherently invasive:

% \begin{quote} I would not be comfortable at all [if someone uses my photo to create deepfake content]. If they don’t take my consent before making that content, I would take it very negatively. And even if they come to me for consent, I would not give it. Whatever the purpose may be, I cannot allow my photo to be used in any content. I am not comfortable, so I cannot give consent from my side. \end{quote}

% These responses underscore the participants' firm stance on the ethical implications of consent and boundaries when it comes to deepfake technology. They illustrate the strong personal and emotional impact of such decisions, and reinforces the need for accountability and respect in the creation and sharing of digital content.

% \subsection{Vulnerabilities of Women in the Cultural Context}
% Participants consistently highlighted how deepfake-related abuse might potentially disproportionately affect women in Bangladesh due to deeply entrenched societal norms, patriarchal structures, and cultural practices. These factors not only make women more vulnerable to reputational harm but also significantly limit their ability to seek help or take action.

% One participant emphasized how easily a woman’s reputation can be tarnished in Bangladeshi society, where such allegations are readily believed without question:

% \begin{quote} Actually, in our community, a woman's reputation is very easily breakable. You can easily talk badly about a woman, and it is readily believed. It harms her reputation terribly, and socially, her image gets torn apart in her family or community. We live in a patriarchal society. In such cases, she becomes a mockery. Maybe people once saw her as a great personality, but after this, they don't take her seriously anymore. They even add extra lines to demean her. These things are extremely common—men, society, and even other women do it. Whether it’s in her family, community, or workplace, she becomes a subject of ridicule, and people feel entitled to talk about her anytime they want. \end{quote}

% Participants also observed that cultural norms grant society and individuals undue access to women’s lives, perpetuating their vulnerability:

% \begin{quote} Definitely, as I said previously, it’s very easy to point a finger at a woman. In some way, we take the liberty of talking about women into our own hands. We feel entitled to talk about her whenever we want. Women are the most vulnerable ones; they are another minority. \end{quote}

% The impact extends beyond social perception. The participants mentioned that it can affect women’s professional lives and opportunities, as societal judgment is often harsh and unforgiving:

% \begin{quote} In corporate domains, these things are seen as extremely bad. It affects her image a lot, and she can be fired even. The treatment you will get from your workplace is different from what a regular guy or girl would get.  \end{quote}

% The societal double standards further exacerbate the issue, where women face harsher judgments compared to men:

% \begin{quote} Women are more vulnerable than men in this sector. In Bangladesh, girls face more pressure to maintain a good reputation than boys. Even if a man faces a deepfake-related issue, the impact is far less severe than for a woman. For a girl, society assumes she must be like that. But if a boy does the same thing, they dismiss it, saying, "Oh, he’s just a boy; let it go." For a girl, they pick it up, share it, and circulate it among friends. It keeps coming up in every situation. Women face this far more often than men. \end{quote}

% The lack of empathy, awareness, and education in the context of digital ethics exacerbates the issue:

% \begin{quote} In our cultural practices, we don’t understand that we should not do such things or how badly it might impact someone’s mental health. We don’t think about these things. We are not empathetic towards each other. That’s why we don’t have the practices or proper social norms, and even in terms of etiquettes, we are lagging behind. This lack of education prevents us from properly navigating the online space. \end{quote}

% % One of our participants described one of her friends' story women often face these challenges in isolation due to the cultural and societal barriers preventing them from seeking help:

% % \begin{quote} Everyone in Bangladesh is a bit conservative, and her parents were quite religious and reputed people. Since she was facing threats, she didn’t have much space to seek help. At the time, cyberbullying awareness wasn’t as advanced as it is now. She didn’t even know that it could be considered a cybercrime. Women in Bangladesh face a lot of these situations. She tried to handle it by herself and didn’t share it with anyone. Instead, she made a deal with them, paying to have the content removed from the internet. \end{quote}

% Participants pointed out how societal norms in Bangladesh differ significantly from those in other countries which limit women’s ability to seek justice:

% \begin{quote} Bangladeshi societal norms are very conservative, especially regarding women. There are many cultural and religious barriers. For example, if a woman’s face or voice is used in a negative context, society will drag her down and ruin her life. In other countries, women might face harassment, but they have access to resources and support, such as cybercrime laws. In Bangladesh, societal norms prevent women from even speaking up, making it extremely difficult for them to seek help. These norms create a very bad impact on their lives. \end{quote}

% These narratives demonstrate how deeply cultural and societal practices exacerbate the vulnerabilities of women to deepfake-related abuse. The interplay of gender discrimination, lack of digital literacy, and societal conservatism creates an environment where women face significant risks and limited avenues for redress.


% These stories illustrate how the lack of awareness and education about digital ethics amplifies the harmful potential of deepfakes. As one participant noted, the limited understanding of privacy, consent, and ethical behavior creates an environment where deepfake-related abuses can thrive, leaving victims without sufficient recourse.


% \subsection{positives}

% \begin{quote}
%     I think that the positive side is more, specially for the purpose of branding, marketing or advertising these things are being very positively used. I think we still haven't gone to that nefty side of it where, I mean from my side if I see then I see the positive sides more in accordance of the use. 

% \end{quote}

% \subsection{talking about deepfakes}

% \begin{quote}
%      In a very funny way yes, like we talk about how it so easy to make a kissing video, but not necessarily about the safeguarding issue of it. It's not necessarily impactful conversation. we talk about the harmful side of it in a very funny or joking kind of way, like see what people are doing these days? Look, what I can do with this app. I mean we talk about this kind of things but the ethical side of it bar moral side of it is hardly talked about in our conversation.
% \end{quote}

% \subsection{familiarity of deepfake}

% \begin{quote}
%      I think in the context of Bangladesh, those of us who have access to the internet, or who have the technical ability to use apps and create content, are not entirely educated about how to use these tools responsibly. We don't understand privacy or consent. We don't understand ethical or unethical issues. We don't know how to behave in cyberspace. This gap in awareness and thought processes means that we are not fully prepared to handle these technologies. I feel like we are not ready for it yet. Again, we don't understand consent or privacy or ethical from unethical. 
% \end{quote}

% \begin{quote}
%     here in Dhaka I live in a very Technology advanced place it's a main point of Dhaka city. Rural area or if we go out side of the Dhaka Metro maybe in Savar the case will be different and if we go even farther in the rural areas or in the suberbens, they have less access to these things or they lack the knowledge to access these things. These things are definitely comparatively less. 

% \end{quote}

% \begin{quote}
%     I am saying is people have become very advanced, they have become very modern and the they stay alert regarding cyber bullying but not everyone can detect, the AI generated fake contents images or whatever that are being created. Because they don't know how to detect these kind of thing.(...) Bangladeshi people definitely use Technology but they are not using it consciously or are not being alert.
% \end{quote}

% \begin{quote}
%     Yes in Dhaka people somewhat understand about the use of AI and how we can use technology to make such contents. They do have some knowledge of it but if we go outside Dhaka they don't even have the knowledge of these kind of things. And their not that developed Technologically, they and even aware much about these Technologies. They are just a user of these. They just use it and sometimes see content that have been created by using this. So because of that what happens is, if something like this happens in Dhaka , and since Dhaka is not that big, if someone faces such incident, you might get to know about this slowly and eventually if the content is real or fake. Because Dhaka community I mean Dhaka city is quite small. But when we go outside of Dhaka, we will see that people are more conservative in those places, and their leg the knowledge of the kind of things. And they have no knowledge or ideas that content might be fake. They automatically believe whatever they see. But they have no idea about how it can be created or manipulated or remade. So in that case I think that how these things are being differentiated in Dhaka or in the Suburban areas of Dhaka. 
%     because of the lack of knowledge or idea what happens is the girl has to face more harassment from the society. They believe that something must have been done by the girl, yes you must have done it! We don't know anything else you must be lying! They just put it on the girl very easily. And obviously she has to face more harassment, abuse and a lot of other things. 

% \end{quote}

% \subsection{sharing photo online/privacy strategies}

% \begin{quote}
%     Absolutely not (comfortable sharing my photo online). Even though because of my professional life and my artist life I have to keep some of it public, but I don't feel comfortable at all sharing my information. Because recently the online harassment has been a big issue. And I have gone through these kind of harassment. Incidence like this has happened to me, because of these reasons I mean I do share but with a constant fear. (...) In some cases I don't even share something online, sometimes I don't even comment publicly online. For the fear of they might trace me back to my profile from that comment and access my information. Nowadays, you can make anything if you want. Some people might figure out that it's a fake thing or someone has made a fake content, but that will take some time, so before that limited time exposure is harassment to me. Even passport size photo, I mean where only your face is visible,  wherever my faces visible that's enough [to make these content].

% \end{quote}

% \begin{quote}
%     in social media, I wouldn't say I am very careful . I don't use fake photos I use my real photos in my social media. 

% I: And beside social media what about dating apps? 
% R: I share my real pictures and real information there as well. 
% I: You are sharing those publicly in the public space? 
% R: Yes, 
% I: Okay, Do you worry about your photos or videos being misused or manipulated? Why or why not? 
% R: Yes definitely I do have, people do this practices for nothing, they use photos to manipulate them. They make a random manipulated picture from an original picture just for fun. In some cases just to defame someone. These practices have grown in number a lot. 
% \end{quote}

% \begin{quote}
%      No one has the public access of my accounts. This basically started because I was a very reserved person. But while I was growing up, I saw that the people who has public profiles they are facing very different kind of problems. Daily people keeps messaging them, they use their profile photos to make different fake profiles to talk with other people pretending to be a real person. i even saw this kind of things happening around me. But in my case what happens is when I post a picture or video or anything like that or make a caption or something like that in that case I usually maintain my privacy. I have selected people in my list, only they can see or access my informations. No one else can. That's how I usually maintain my privacy. 
% I: And what about your dating profile, if you have one? In that case do you maintain the same privacy? 
% R: No, that's very unfortunate but when one opens up a dating profile, then people around you or living around you can see that this person exists. In that case I am breaching my own privacy with my own hands. My photo my information can be seen by everyone there. But in that case what we can do is share minimum information that cannot be used against me. A photo like sharing a photo like this or creating a Bio like this, you can set information like this I think. 
% I: Okay, even after having a customized profile or a locked profile, do you ever worry that your photo or your information can still be misused or manipulated by anyone? [Q7:VVIQ]
% R: Yes, that's a very realistic possibility. If I can share a small story, one of my friends had their profiles locked and Secured them just like me.but they got in an argument with another friend, so as a result what they did was they took a screenshot of their profile, also all of the comments on their social media and they made a public post about them with those information. The post said that the girl is like this and that and she has done this and that, even her address was leaked through that post. It mentioned where she lived and whatever she spoke about. And after that I also heard that, some people also give her threats that they know where she lives, so they will come to her house and beat her up in her own home. So these kind of things also do happend even though you have a locked profile. I think in the world of social media you can never be more alert. You can never be enough alert. You always have to be more cautious or alert, if you are sharing your photo or your information in a social platform or media there is always some kind of risk of something happening. You cannot always be sure that nothing will happen however locked your profile is. If Other people have access of your social media that means your photo or video might get easily misused. So in that case something like that can easily happen. 
% I: So you do have that kind of worry in your head? 
% R: Yes 

% \end{quote}

% \subsection{harassment}

% \begin{quote}
%     One of my friends had shared some photos with her boyfriend. Later when they broke up and they swiped photos of her with something else. Then the girl created an expose post about the guy like how he tortured her. Then from the guy's side he shared some contents like these online to bully the girl. So, I saw the story where the girls pictures were manipulated. 
%     People has done a lot of mockery on this. A lot of online joke has been going on between her own friends let alone others. Even in conversations this came up as the topic where her peers talked about how a content has been made about her, in a very disrespectful and funny way.
% \end{quote}

% \begin{quote}
%      one of my cousin who was an influencer on Instagram, so she got bullied or harassed in her inbox a lot of times. She was used to it at some point. But at a point a very viral content was released on social media where they to only her face from a picture and used it in a pornography. And later she was being threatened with the content as well. Because people did not get that the content is fake. Maybe she knows it and I understand it but people have no way of knowing if it's real or fake. So because of that they had to face a lot of threat as well. She also had to pay a fine for it as well as far as I can remember. So that the content gets deleted. (..) it was someone from her follower list. Some guy from her follower list who wanted to initiate a romantic relationship with her but as she refuseed later and incident like this happen with her. 

% \end{quote}

% \subsection{vulnerabilities of women in the cultural context}

% \begin{quote}
%      Actually in our community a women's reputation is very easily breakable. You can easily talk about a woman talk bad about her. It is easily believable and it gets accepted as the girl might have done this surely. It harms her reputation terribly plus socially her image gets torn apart a lot to her family or her community. We live in a male dominated society or a patriarchal society. So in this cases what we can see in accordance with the social standing is that she turns into a mockery. Maybe they looked at her as a great personality but just because this happen they don't take her seriously anymore. Or if they are talking about her they add extra one of two lines to demean her. These things are extremely common in our society. Men do this all the time but society does that as well and in some cases other girls do it too. So, in terms of her family or community or reputation or if I talk about the work space everywhere she turns into a Mockery, and its like they have access to talk about her anytime they want and in any way they want. 

% Definitely it can affect her work as well. In fact in corporate areas these things are counted as extremely bad and effects her image and how she is and also what her designation should be. In this cases her social standing matters a lot. Like if you are a very famous artist, the treatment you will get from your office, a regular guy or regular girl would not get the same treatment. Because the social standing ads a value to it. 

% \end{quote}

% \begin{quote}
%     Definitely, as I said previously it's very easy to point a finger at a woman. And in some way we take the access of talking about a woman in our own hand, we can talk about her if we want anytime. So definitely they are the most vulnerable ones, they are another minorities. 

% \end{quote}

% \begin{quote}
%     Yes, in our cultural practices we don't have things like um... We don't understand that we should not do this kind of things or this is not right or this might impact someone's mental health very badly. We don't think about these things, we are not empathetic towards each other. That's why we don't understand. So definitely we don't have the practices we don't have moderate social norms and even if I talk about etiquettes, in that cases we are lagging behind. We don't have the proper education in US about these things that's why we cannot properly execute on the online space. 
% I: And the impacts that it does it can be in any kind of way. whoever the victim of the deepfakes are if i may say so, does the impact of such incident very because of other Bangladeshi cultural practices and social norms. For example in foreign countries they might behave in a certain way if faced by these kind of incident but as opposed to Bangladesh, the Bangladeshi society my react to a different way because of how our social and cultural practices are. 
% R: Yes definitely they are more secured than us. 
% \end{quote}

% \begin{quote}
%     The situation was something like Appu, everyone in bangladesh is a bit conservative and her parents are quite religious and reputed people. So in that situation since she was going through and facing a lot of threats, she didn't have much space to go to someone seeking for help. Because then things like cyber bullying were not this much advanced as now it is. Because of that she didn't even have the knowledge that it would be considered as a cyber crime. That's because of the lacking of awareness. Usually women in Bangladesh face a lot of these. So what she did was she tried to handle it by herself. She didn't share it with anyone at that time. She just kept inside her head and tried to figure out a solution by herself. So she didn't take any step or didn't take any legal help, instead.. she made a deal with them regarding a payment to remove the content from online. 
% \end{quote}

% [impact]
% \begin{quote}
%     R: Yes definitely I would say women are more vulnerable than man in the sector. Of course there are reasons behind this. Because in Bangladesh we see a lot of discrimination between boys and girls. The girls have the pressure to maintain a very good reputation for the society rather than the boys. We see that a man is faced with the issue of any deepfake related content way less than a woman. It has reasons behind it as well. even if they are facing the issues of deep fake, that issue does not create as much of a negative impact on the men as it does for the women. Because we see that in Bangladesh perspective, a girls reputation or there humility or keeping them inside the house what the content they are creating all of these face a very negative comment or perspective from the society. Whatever the content maybe, they agree that may be the girl might be like that. But if a boy does the same thing they will say that oh he is just a boy, let it go. I have seen a lot of these happening around me where they say oh he is just guy, let him go! But if it's a girl they will pick it up and share it among themselves they will circulate it and talk about it with their friends. They will keep bring it up in every situation. These things keep happening always so in that case I think women are much more than a man. 
% I: Okay,Apu you have already mentioned that society is giving a man the privilege of letting go so in that case I want to ask you another question that,Do you think the impact is more related to social norms and religious/cultural practices and can it vary depending on different areas? 
% R: Yes definitely it does create an impact. Because in other countries, because of the mass population of them it's hard to know everyone and their is a space for not knowing a person. And the people in other countries have different mentality than our Bangladeshi people. They are more developed. So in that space if I have to say so I am not interely sure if they are recognising the AI related content or understanding if a content is fake or not. But in Bangladesh we don't usually Count these things. To check if it if a content or not. But what Bangladeshi people does is, the effect that are created through deep fake.. 
% I: Apu please in your own words, no issues . Should I repeat the question?
% R: Yes please 
% I:Do you think the impact is more related to social norms and religious/cultural practices and can it vary depending on different areas? 
% R: Yes Bangladesh societal norms are very conservative. Specially when it comes to women, because they are many cultural barriers or religious barriers. In almost every angle the society norms teachers that if a women's face or a woman appears on a screen, these things have a lot of barricades. In that case is a content as exclusive as such gets out, or if her picture or voice is being used to create a negative content or a voice over, in that case that society will down right drag her down and ruin her life. So, in that case I think the society norms do impact on the life of the person. Because in other countries I don't think the girl has to go through these much of harassment, or face so much pressure or negative comments. In other countries I think if a girl is facing a deepfake related issue then she gets the help of some Technology as well. The steps you have to take under cyber crime, maybe she is taking those as well. But in Bangladesh what happens is ,because of the societal norms the girl cannot even speak up and late anyone know that these kind of thing are happening with her. Since she can't even speak up about these things, you can imagine how tough it is for her to get some help. I think the society norms create a very bad impact like this on her. 

% \end{quote}

% \subsection{Checking Authenticity}


% \begin{quote}
%     I: Okay, Apu. What steps, if any, do you take to verify the authenticity of content you see online (e.g., news, videos, or images)? 
% R: Not always not always. The images that impact me emotionally, then I usually don't check. But in regards to fact based data, I definitely check for authenticity. 
% I: Is that different for your work space and other spaces? 
% R: Definitely it's different. In professional life there is no emotion involved. Whatever I find online I check The authenticity of the content or verify the content. But on personal level, a lot of images i get to see in online spaces are personally triggering or emotionally triggering, that I don't understand if they are edited or not always. I don't even always have the head space to check those. 

% \end{quote}

% \begin{quote}
%     I am saying is people have become very advanced, they have become very modern and the they stay alert regarding cyber bullying but not everyone can detect, the AI generated fake contents images or whatever that are being created. Because they don't know how to detect these kind of thing.
% \end{quote}

% \begin{quote}
%     R: No, no such thing happened actually. Instead if a viral News or something that is happening in our country, if I come across such news regarding the issue however unrealistic it may be, it easily gets spread around and reaches everyone instantly. Like do you know what happened? See? this has just happened. But no one is checking if that incident really happened or not. So in that case there is not much scope of verifying any news. And if something like that happens that where it is being circulated from, for example something like that happened a while back, people kept asking why did you get? it what's the source? Because so much contents regarding deepfake was scattered around everywhere, or being shared that people got annoyed at that point asking for the source of it. So regarding an authentic source now we see that, at least my Peers do not believe in a content that does not have an authentic source. Even if it get share they are like ...wait, let me check The authenticity first if true or lie. Maybe them they do a little research around them to check if that really happened or not, but the tag of being verified that it is in fact authentic nothing like this exist I think. If you tag it as authentic then it get easy to recognise if a content is real or not. But normally there is not such process. 
% I: Ok, when you mention that you are asking your Peers or checking the comment section that also counts as a verification process. So you do go through the verification process of those news. 
% R: Yes yes. 

% \end{quote}

% \subsection{Consent and Setting Boundaries}

% \begin{quote}
%  I: Okay, To which extent would you feel comfortable with a content being used as deepfakes (shared by family member/ friends/partner/stranger on a private/public online space) and where do you draw the line of being fun and being harmful? 
% R: Family member, if you friends maybe. Maybe my partner. 
% I: And what about sharing those in private spaces? How comfortable would you be? 
% R: I would not be comfortable at all. It can be in a very inner space like it can be sharedin my inbox or in my group chat, to that extent I think it is fine for me. No problem. But those people has to be very close to me of course. 
% I: Okay, and what if we talk about public platform? 
% R: In public platforms, not at all. You have to take my consent first.    
% \end{quote}

% \begin{quote}
%     I: Ok,To what extent would you feel comfortable with a content being used as deepfakes (shared by family member/ friends/partner/stranger on a private/public online space) and where do you draw the line between being fun and being harmful? 
% R: I would not be comfortable at all. If they don't take my consent before making that content, I would rather take it very negatively. And if they come to me for consent I would not give them the consent. Whatever the purpose maybe I cannot allow my photo to be used in any content. I am not comfortable, so I cannot give them any consent from my side. 

% \end{quote}

% \subsection{fun or harm?}

% \begin{quote}
%     at first if used to be a fun thing for me when it was used mostly for entertainment purpose. But now a days people are using these to maybe poke someone or to Bully someone or to Harris someone or in some cases to create political issue with someone. A lot of such contents are coming up which are not just for entertainment purposes. It is almost used as a weapon nowadays for example, they will take there Voice and modify it in a different speech or someone is saying something but they are lip sync is different where you can see that the speech is coming of differently. So things like that used to be entertaining before but nowadays it has become very risky and since it is being used to Bully someone or against someone, and a lot of people are being targeted through this so for me the idea of the fake has been kind of a negative idea in retrospect. So I don't like the use of deep fake that much. I think it is mostly used to harm people nowadays. 

% \end{quote}

% \begin{quote}
%     R: What I think is the deepfake content creating has the most affect on the person's mental health. Because suddenly if a fake content comes out which they didn't do or didn't say or wasn't involved in any kind of way, when they see themselves in a situation like this... And specially if it's not done for an entertainment purpose. Instead it is getting created in a very attacking way. So on suddenly things like this come on to a human being then they get mentally torn apart, and when they are family is shown that such kind of thing are faced by them like see these kind of things have happened with me, then the question is always race against the women. Did you really do this? Be truthful, did you? Then automatically the scope of them getting help gets reduced. So this kind of things happen. And when a society gets to know about things like this, her family get pressurized to control their daughter or sister. Why don't you control her? She is doing this and that! They tag her as bad. So because of things like this we see that the girl is accused for everything. And in workplace definitely, people talk behind her back. Or gossiping about.. see? what happened to that girl? Now a days everyone uses Technology and even with a button press you can share anything and everything. So the thing never stays in one place. It gets spreaded everywhere very easily. That's how everyone gets to know about almost everything. Since everyone is getting the access to know about these things in that case, the girl has to face these kind of situation unfortunately. 
% I: So you are talking about a very negative impact ultimately? 
% R: Yes very very negative impact.
% \end{quote}

% \subsection{Deepfakes: Moral and Legal?}

% \begin{quote}
%     I: Okay, Do you think deepfake misuse is primarily a moral issue, a legal issue, or both? Why? 
% R: Yes it is in both ways. I have already talked about the moral issue of it. The ethical perspective I talked about. So it definitely direct toward moral issue. And and two think about the legal issues, yes cyber harassment is a real harassment. It definitely effects a person mentally and physically both. It harms them. So definitely it is a legal issue. Legally this thing needs to be stopped. Legally we need to have charges for this. 

% \end{quote}

% \subsection{Legal Help}

% \begin{quote}
%     I: Okay, Do you think deepfake misuse is primarily a moral issue, a legal issue, or both? Why? 
% R: Yes it is in both ways. I have already talked about the moral issue of it. The ethical perspective I talked about. So it definitely direct toward moral issue. And and two think about the legal issues, yes cyber harassment is a real harassment. It definitely effects a person mentally and physically both. It harms them. So definitely it is a legal issue. Legally this thing needs to be stopped. Legally we need to have charges for this. 

% \end{quote}

% \begin{quote}
%     Their hasn't been a proper policy created to tackle or handle these kind of situation. We need to do more advocacy on this topic regarding policy making. What happens in our country is, after you pass a law, the laws don't get properly implemented. So we should be more attentive in terms of law enforcement. We can't even implement the existing laws properly. So before making a new law we should work on the existing laws. Like we can make one or two laws addressing this situation, those that are important, I mean one thing at a time. But these things should be constantly updated. 
% \end{quote}

% \begin{quote}
%      The laws should address all kind of genders. Because the gender based activities are more in our country. It's not like we behave same with all genders equally or treat them equally. So since we look at gender differently in our own practices, so our laws and policies should reflect the same and become more gender sensitive. That's what I think. And we need the feminist angle for this. It doesn't necessarily have to be a feminist organisation, but if they can take the calls then they should. It's not like they can't think gender sensitively. 
% \end{quote}

% \begin{quote}
%     I: Since you talked about authorities, Do you think law enforcement and other authorities are prepared to handle deepfake-related cases? Why or why not? 
% R: No they are not prepared, they are absolutely not prepared for it. Because they still are not active regarding cyber space harrestment. And a new trend or a new concept like deep fake, I don't think they are still fully aware or ready to handle cases like this. What they don't have enough tool to prevent these kind of content. 
% \end{quote}

% \subsection{Design Recommendations}

% \begin{quote}
%     I:What kinds of legal, social, or technological measures would you like to see implemented to address deepfake misuse? 
% R: We should make something I mean what I think is we should make a tool that would be attached to all the platforms and whenever a deep fake like this occurs, it will remove that instantly. It will identify the deep fake as fake news or a fake photo, so you cannot publish it. You have to delete it otherwise your account or profile will be blocked or deleted or banned. We should make it too like this and it will be Incorporated on every social media or other platforms. Just to identify the deep fake, fake photos or fake videos or fake news. Like we have rumours scanner, I am talking about something like that. 

% \end{quote}

% \subsection{creating awareness}

% \begin{quote}
%     If I have to talk on the deep pics or about online safety, we actually don't have any online safety. We don't know a lot of measurements on how to secure ourselves or people cannot access our personal information. How to profile lock or save our information. So we need to talk more and there should be more conversations on the topic or do more activities. What I think is the world we live in right now is entirely Technological. We are very dependent on the technology. So we need to talk a lot about this topic made be on education level or in practice or in official space. Training, grooming I mean however it may be we should talk more about this topic. 

% \end{quote}

% \begin{quote}
%     Here, what I think is, bangladesh government can play a very effective and impactful role. I don't know if you remember before acid throwing was a very big issue in our society. Whatever happens people would get aggressive and throw acid made be a rejection from a love interest. I don't know if you remember the government specially from the channel BTV, they started a huge campaign against this . They portrayed how a acid throw a perpetrated will get punished. They created a massive campaign on this. Banners posters wall painting TV Advertisement and a lot of those. In that time people like myself got really impacted. And also if I may say so, is song that came out in a campaign which we still seeing to this day against drug abuse, ek song by Kabir Suman, "Sudhu jontrona, Bachao jibon guli, Bachao chetona". I mean this kind of initiatives stay with you. Even after 10 or 15 years we are still singing the songs. Because the things were really impactful. And if you look at the statistics of it, after those campaigns the acid incident and drug abuse got lessened after 2006 or 7 because of these campaigns. So here our government can play a very impact full and effective role if they have budget to address this kind of issues. Okay? And they have to get smart with it as well. We are talking about smart Bangladesh aren't we? This is high time to address these things. And that's how we will be able to educate our people. And definitely it's a fact about our own personal practices as well. But media can play a very big roll in this space. Media make people talk. What you want to talk about it is decided by the media. 

% \end{quote}

% \begin{quote}
%     I: Okay Apu when you are talking about media involvement, would you incorporate different social media's or platforms here as well? Or what platforms or medias according to you, could we use to circulate the kind of messages or informations? 
% R: Firstly Facebook, YouTube because a lot of news I watch only on YouTube now a days. And people who have access to TVS or watch them regularly like the older generation. 
% I: Or if you want to add anything area wise ?
% R: Whoever has what ever kind of access in their area. But nowadays even the rural areas have access to smartphone. Smartphones have been very accessible so they have the access. 
% I: Okay, I get it. We are almost at the end of our interview. As you have already mentioned the government,How can society, as a whole, better address the risks posed by deepfakes? 
% R: As a society? This is a very tough question because our society is very scattered now. We have a online society. I am in how to address this kind of things.... Regarding these I will still say media make people talk. Media surfaces the Trends or the viral issues, we usually talk about the talk of town newses. Then we start a conversation among ourselves. That's how we can address some of these incidents. Some kind of event or festival can be arranged. 
% I: Since we are talking about more awareness or sensitization what I want to ask is would any academic intervention or training help to improve or make them aware of the risk in your opinion? 
% R: I think from younger generation to the older one everyone should learn about these things. For example, those who are working in ICT or working in the field of IT, who are working in the sensitive issues, they also need proper training may it be online or somewhere overseas. And also in education level starting from the children and to the bigger audience, where we have topic of science or Technology, they are should be more talk about these kind of issues. That's how we have to go into the education sector, we can incorporate them in our academic book as well. Or we can have courses on them or different workshops different seminars conference or dialogues, like we can arrange seminar where the agenda is basically how we can prevent the deep fake misuse contents or something like this. For where we can identify a deepfake content, how to do it. We have two work in this from every angle, may it be on education level or in the society. 

% \end{quote}



==> intro-old.tex <==
\section{Introduction}
The advent of deepfake technology, a product of advancements in artificial intelligence (AI) and deep learning, has revolutionized the generation of synthetic media, such as images, videos, audio, and text. By enabling the seamless transfer of one individual's voice, image, or movements onto another, often without consent, deepfakes have sparked both excitement and apprehension. While this technology offers creative possibilities in entertainment, education, and creative industries, it simultaneously poses significant ethical, societal, and legal challenges. The growing sophistication of deepfake content has blurred the lines between reality and fabrication, which has led to potential consequences for trust, privacy, and societal norms.

The term ``Deepfake” first appeared on the Reddit platform in
2017. The user of the same name, ``deepfakes", was the first person to publicly post deepfake videos in which the faces of prominent women were inserted onto the heads of actresses in adult video clips without their consent. Their username was made up of the two terms ``Deep Learning" and ``Fake" and is the basis for the naming. As the codes for creating the deepfakes were shared, there was an immense increase in such content (Kietzmann et al., 2019). Since then, its application has expanded, raising concerns over its role in misinformation, political propaganda, fraud, and image-based harassment and abuse. The State of Deepfakes 2019 Landscape, Threats, and Impact found that 96 percent of deepfakes were non-consensual sexual deepfakes, and of those, 99 percent were made of women. (Dunn, 2021) In 2018, the top deepfake porn site contained less than 2,000 deepfake pornographic videos, but this number grew to 13,000 by 2022, and the site is now attracting 16 million viewers per month. (Mft, 2023). The democratization of AI tools has led to this technology’s integration into everyday contexts, which highlights the far-reaching implications of deepfakes in eroding trust, damaging reputations, and challenging societal values - where its impacts remain underexplored.

While much of the current discourse around deepfakes focuses on technological advancements in creation and detection, the societal and cultural implications of this technology, particularly in non-Western contexts, are underexamined. For example, in patriarchal societies like Bangladesh, deepfakes are increasingly used as tools for harassment, defamation, and exploitation, which disproportionately affect women. The lack of adequate regulatory frameworks, limited digital literacy, and cultural stigma further exacerbate these issues. Despite the pressing nature of these challenges, there remains a paucity of empirical research on how deepfakes are perceived, experienced, and discussed in such regions.


This study seeks to address this gap by exploring the perceptions of deepfake technology among Bangladeshi women. By centering their voices, the research investigates their awareness, emotional responses, and the socio-cultural implications of deepfakes in their lives. This investigation not only provides critical insights into the localized impacts of deepfake technology but also highlights the need for interdisciplinary approaches to develop culturally sensitive solutions for mitigating harm. By examining deepfakes through a human-centric lens, this study contributes to a broader understanding of the complex intersection between emerging technologies and societal vulnerabilities.



==> lit-old.tex <==
\section{Background and Related Work}
Detection niye onek kaj hoise. Legislation and regulation niye kaj hoise
% \\

The authors Gamage et al. define deepfakes as follows: Deepfakes are the application of deep learning methods to generate fake content—usually video, images, audio or text. The quality of content created by deepfake technology is improving, making it indistinguishable from real content. This involves transferring one’s voice, video, or image to another to reflect the original person, mostly done without consent. (Gamage et al., 2022, p. 2) The understanding of what exactly deepfakes are, differs in two ways: either there is talk of the original meaning, or it has adopted a meaning the term has received over time. Moreover, the definition of Gamage et al. (2022) is broadly formulated and is closer to a definition of synthetic media, which could be seen as an umbrella term for all types of media, such as virtual reality and advanced digital-image creation and not just AI-generated or manipulated videos (Whittaker et al., 2020). Deepfake technology by origin is actually a subcategory of synthetic media production and is the swapping or replacement of faces, facial features or expressions by AI. The replacement of whole bodies and the manipulation and creation of audio files like speech was developed at a later point of time and is now also considered to be deepfake media. Hence, even though the origin of deepfake is based on the manipulation of faces in visual content, it is now used interchangeably with synthetic media, AI-generated media, generative media, and similar terms.

As the potential implications of deepfakes have become more evident due to progress in AI technology, there has been an increase
in research studies focused on deepfakes []. While most studies
focus on deepfake detection [], i.e., developing algorithms and models for this task, and legal implications of deepfake technology, studies exploring how deepfakes are perceived have been nascent. The deepfake phenomenon must be positioned within the sphere of society, culture and values, and should be examined under the lens of the contexts of its uses (or potential uses), along with its effects. Currently, researchers indicate that deepfakes will have implications in law and regulations, politics, media production, media representation, media audiences, and overarching interactions in media and society []. With the commercial development of AI applications such as FakeApp (https://www.faceapp.com/), Deepfake Web (https://deepfakesweb.com) and Zao (https://zaodownload.com/) or audio deepfake apps such as Resemble (https://www.resemble.ai), and Descript (https://www.descript.com/overdub) as well as with the use of synthesized text [], it is evident that attacks involving human reenactments and replacement are emerging. Cyber security reports in 2019 predict 96\% of all deepfakes to be pornographic [] and other forms of harmful outcomes []. In addition, research reveals alarming concerns over developments in deepfake child pornography [18] or applications such as DeepNude where algorithms remove clothes from images of women []. Furthermore, the current platforms’ business model is contentdriven and use incentives to increase the number of views and likes. Platforms such as Facebook, Twitter, YouTube, TikTok, and Reddit are all competing for users’ attention []. Due to signi!cant monetary incentives, content creators are pushed into presenting dramatic or shocking videos, where potential deepfakes may draw the attention of the public []. Although some research suggests that the increased proliferation of deepfake videos will eventually make people more aware that they should not always believe what they see [], much empirical research is essential to understanding the impact and estimating the potential damage where interventions are needed before deepfake causes harm.

Although limited research can be found providing social evidence of how people react or what they understand when they see deepfakes, a study conducted in 2020 using a sample of 2,005 UK citizens provides the first evidence of the deceptiveness of deepfakes []. In published articles discussing deepfake societal implications, the authors have brought many anecdotal shreds of evidence leading to the prospect of mass production and diffusion of deepfakes by malicious actors and how it could present extremely serious challenges to society []. Since the social perspectives are based on “seeing is believing” or “a picture is worth a thousands of words”, images and videos have much stronger persuasive power than text; thus citizens have comparatively weak defenses against visual deception of this kind []. Particularly the research by [] investigated how people can be deceived by political deepfake, and it turns out that society is more likely to feel uncertain than to be completely misled by deepfakes. Yet the resulting uncertainty, in turn, reduces trust in the news on social media. The societal implications of deepfakes can be easily grounded when we understand how people interact with such technology. Overall, considerable research has highlighted that deepfakes are likely to attack in the spheres of political disinformation and pornography. One of the latest research studies indicates the likelihood of sharing deepfakes based on individuals’ cognitive ability, political interest and network size []. Although deepfakes are relatively new and risks have yet to be seen, many reports show that deepfakes have the potential to influence multiple sectors of society such as the financial sector which relies on information, politics, national and international security []. They may even threaten private lives by revenge porn and faked evidence used in legal cases resulting in distress and suffering []. Although many in the !eld of communications, media, and psychology try to understand the impact of deepfakes, areas such as human-computer interaction and human-centric designs have sparsely been covered in exploring deepfake effects on society. To highlight, we found only nine research articles from the search term “deepfake” in the prominent conference on Computer Human Interaction conference (CHI). Of the nine articles, only two articles involved perceptions of deepfakes’ impact on society. Of those two, one research article conducted experiments focusing on psychologically measurable signals which could be used to design tools to detect deepfake images []. The other study more importantly addressed how human eyes detect deepfake while providing implications of a designed training for distinguishing deepfakes, especially in low literate society []. By far one of the most factual evidence of widely known deepfake effect—revenge porn is described in an article from CHItaly. Their research provides an expert analysis of the process of reporting revenge porn abuse in selected content sharing platforms such as image and video hosting websites and pornographic sites. In a search for a way to report abuse by revenge pornography using deepfakes, they found serious gaps in technology designs to facilitate such reporting. This research provides a view of current practices and potential issues in the procedures designed by providers for reporting these abuses []. With all of the research, it is evident that deepfakes could damage individuals and society. Prevention and detection may be one way of looking at it. The design of digital technologies will play an important role in reacting to any social issue cause by deepfakes and interdisciplinary approaches must be taken to address these issues. In this research, we examine the perceptions of Bangladeshi women related to deepfakes and identify emerging threats while proposing recommendations integrating changes in technological and societal behavior.



